Zerrow: True Zero-Copy Arrow Pipelines in Bauplan

Bauplan is a FaaS-based lakehouse specifically built for data pipelines: its execution engine uses Apache Arrow for data passing between the nodes in the DAG. While Arrow is known as the "zero copy format", in practice, limited Linux kernel support for shared memory makes it difficult to avoid copying entirely. In this work, we introduce several new techniques to eliminate nearly all copying from pipelines: in particular, we implement a new kernel module that performs de-anonymization, thus eliminating a copy to intermediate data. We conclude by sharing our preliminary evaluation on different workloads types, as well as discussing our plan for future improvements.

==> Makefile <==
MAIN      = main
SRCS      = *.tex 
TARG      = $(MAIN).pdf


all: $(TARG)

pdf: $(SRCS) $(MAIN).bbl
	source ./SourceMe ; \
	pdflatex $(MAIN)
	source ./SourceMe ; \
	pdflatex $(MAIN)
	#cp main.pdf ~/Dropbox/Documents/

$(TARG): $(SRCS) $(MAIN).bbl
	source ./SourceMe ; \
	pdflatex $(MAIN)
	source ./SourceMe ; \
	pdflatex $(MAIN)
	touch $(TARG)
	#cp main.pdf ~/Dropbox/Documents/

bib: $(MAIN).bbl bib.tex

$(MAIN).bbl: $(MAIN).aux
	source ./SourceMe ; \
	bibtex -min-crossrefs=100 $(MAIN)
	# The below line is commented because usenix started checking
	# formatting for references also -- running redo-bib would 
	# squish the references without space to which the format 
	# checker would complain! 
	#./redo-bib.csh $(MAIN)

$(MAIN).aux: $(MAIN).tex
	source ./SourceMe ; \
	pdflatex $(MAIN)

clean:
	rm -f $(TARG) *.aux *~ $(MAIN).log $(MAIN).bbl $(MAIN).blg $(MAIN).out $(MAIN).dep

.SECONDARY: $(DVI)


==> fig-tex/eval_parallel.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/eval_parallel_load.eps}
%     \caption{\textbf{E2E Throughput of Parallel Load Functions with 50\GB\ Memory Limit.}
%         The workload is a load workload which loads 0.5\GB\ parquet file into Arrow in-memory format with a size of 4\GB\ and outputs Arrow IPC format. DeAnon\_noswap and Baseline\_noswap are the experiments with no swap space, terminating at 9 and 6 parallel functions respectively. (How can I plot better to show that? Maybe in 2 graphs?)}
%     \label{fig:parallel-load}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/eval_parallel_load_major_faults.eps}
%     \caption{\textbf{Number of Swaps of Parallel Load Functions with 50\GB\ Memory Limit.}
%         The workload is a load workload which loads 0.5\GB\ parquet file into Arrow in-memory format with a size of 4\GB\ and outputs Arrow IPC format. Y-axis is the number of swaps (in the unit of os pages) during the workload.}
%     \label{fig:parallel-load-swap}
% \end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_parallel_execute.eps}
    \caption{\textbf{E2E Throughput of Parallel Computation-heavy Functions with 50\GB\ Memory Limit.}
        The workload is a computation-heavy function that use transforms 1\GB\ data from the input to 1.4\GB\ output. X-axis is the number of parallel executions and y-axis is the thoughput.}
    \label{fig:parallel-compute}
\end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/eval_parallel_execute_major_faults.eps}
%     \caption{\textbf{Number of Swaps of Parallel Computation-heavy Functions with 50\GB\ Memory Limit.}
%         The workload is a computation-heavy function that use transforms 1\GB\ data from the input to 1.4\GB\ output. X-axis is the number of parallel executions and y-axis is the number of swaps during the workload.}
%     \label{fig:parallel-compute-swap}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/eval_parallel_two.eps}
%     \caption{\textbf{E2E Throughput of Load and Compute Functions with 50\GB\ Memory Limit.}
%         The workload is the sequential execution of the functions in Figure\ref{fig:parallel-load} and Figure\ref{fig:parallel-compute} X-axis is the number of parallel executions and y-axis is the thoughput.}
%     \label{fig:parallel-combine}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/eval_parallel_two_major_faults.eps}
%     \caption{\textbf{Number of Swaps of Load and Compute Functions with 50\GB\ Memory Limit.}
%         The workload is the sequential execution of the functions in Figure\ref{fig:parallel-load} and Figure\ref{fig:parallel-compute} X-axis is the number of parallel executions and y-axis is the number of swaps during the workload.}
%     \label{fig:parallel-combine-swap}
% \end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_parallel_load_v2.eps}
    \caption{TODO}
    \label{fig:eval-parallel-load-v2}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_parallel_two_v2.eps}
    \caption{TODO}
    \label{fig:eval-parallel-two-v2}
\end{figure}


==> fig-tex/eval_schedule.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_schedule_overcommit.eps}
    \caption{\textbf{E2E Latency of Load and Compute Functions with different overcommit percentage.}
        The workload is the same as in Figure\ref{fig:parallel-combine}. Memory limit is 50\GB. X-axis is the totla number of functions and y-axis is the latency.}
    \label{fig:schedule-overcommit}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_schedule_active_eviction.eps}
    \caption{\textbf{E2E Latency of Load and Compute Functions with Different Eviction Methods.}
        The workload is the same as in Figure\ref{fig:parallel-combine}. Memory limit is 50\GB. X-axis is the totla number of functions and y-axis is the latency.}
    \label{fig:schedule-active-eviction}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_schedule_complicated_overcommit.eps}
    \caption{\textbf{E2E Latency of Column Adding Workloads with different overcommit percentage.}
        The workload is the same as in Figure\ref{fig:add-column}, each chain containing 10 functions and 1 to 20 chains are run. Memory limit is 50\GB. X-axis is the totla number of functions and y-axis is the latency.}
    \label{fig:schedule-complicated-overcommit}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_schedule_complicated_eviction.eps}
    \caption{\textbf{E2E Latency of Column Adding Workloads with Different Eviction Methods.}
        The workload is the same as in Figure\ref{fig:add-column}, each chain containing 10 functions and 1 to 20 chains are run. Memory limit is 50\GB. X-axis is the totla number of functions and y-axis is the latency.}
    \label{fig:schedule-complicated-eviction}
\end{figure}


==> fig-tex/eval_thread.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_parallel_two.eps}
    \caption{\textbf{Overall Latency of Load and Compute Functions with 50\GB\ Memory.}
        The workload is the sequential execution of the functions in Figure\ref{fig:parallel-load} and Figure\ref{fig:parallel-compute} X-axis is the number of parallel executions and y-axis is the throughput.}
    \label{fig:eval-thread}
\end{figure}

==> tex/design3.tex <==
\beforesect
\section{\zc{} Design}
\label{sec:design2}
\beforesect

We introduce \zc{}, a new platform that uses shared Arrow data to efficiently pass intermediate data with minimal copying and duplication. \zc{} uses a mix of existing techniques (\textit{share mounting} and \textit{limit dropping}) and novel techniques (\textit{shared deserialization}, \textit{de-anonymization}, \textit{resharing}, \textit{dictionary sharing}, and \textit{IPC inspection}) to overcome the challenges we have described (\S\ref{sec:challenges}). We provide an overview of \zc{}'s major components (\S\ref{sec:arch}) and then explain how we achieve independent code execution (\sref{sec:design-sandbox}), intra-node copy avoidance (\sref{sec:design-sharing}), and sharing-aware resource management in detail (\sref{sec:design-rm}).

\beforesect
\subsection{\zc{} Overview}
\label{sec:arch}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/arch.pdf}
    \caption{\zc{} Architecture and Write Path}
    \label{fig:arch}
\end{figure}

Figure~\ref{fig:arch} illustrates \zc{}'s architecture and four running DAGs (1-4), most of which are using Parquet files as a source. Each square represents a node in a DAG, and shading indicates a node is running or completed.  Intermediate Arrow data (``\textit{A}s'') is passed via shared memory between nodes.

\zc{} runs each node in a container called \textit{node sandbox} to achieve independent code execution while sharing data (\textbf{Challenge 1}). These nodes loads/generates data through a Shared IPC library (\textit{SIPC}) that uses de-anonymization (\textit{KernelZero}) to achieve intra-node copy avoidance (\textbf{Challenge 4 and 5}). \zc{}'s \textit{Resource Manager (RM)}
 examines node dependencies in DAGs to performs caching of deserialized data (\textit{DeCache}) to remove duplication between different nodes and DAGs (\textbf{Challenge 2}). \textit{RM}
retrieves detailed dependency information of intermediate data to the actual physical data by \textit{IPC inspection} (\textbf{Challenge 6}) for better caching and scheduling decisions. Under memory pressure, \textit{RM} performs evictions with the knowledge of dependencies and adopts a new eviction mechanism called \textit{adaptive eviction} (\textbf{Challenge 3}).

\subsection{Independent Code Execution}
\label{sec:design-sandbox}

In order to achieve data sharing and independence between nodes in terms of code resources (\textbf{Challenge 1}), each process runs in its own container, called a \textit{node sandbox}, and all the containers mount a common in-memory file system for sharing data.  This \textit{share mounting} technique is a standard containerization feature (\eg{}, a Docker {\tt --ipc=host} option provides such a mount).

\subsection{Intra-Node Copy Avoidance}
\label{sec:design-sharing}

\zc{} achieves intra-node copy avoidance for intermediate data sharing (\textbf{Challenge 4}) by de-anonymization that converts anonymous memory to shared memory without copying, and input-output sharing (\textbf{Challenge 5}) by resharing that detects sharing of data between inputs and outputs and points outputs to corresponding inputs.

Figure~\ref{fig:arch}b illustrates \zc{}'s write path: (1) the RM allocates memory to start a new sandbox, passing in references to input data, if any.  (2) Inside the sandbox, a \textit{share wrapper} invokes the provided user code.  That code returns Arrow data back to the wrapper. The Arrow data may have been generated by any package using any Arrow implementation, so the data is unlikely to already reside in shared memory.  Instead, the Arrow data will usually reside in \textit{anonymous} memory (\ie{}, memory not backed by a file). This is unfortunate, as processes in downstream nodes will need a reference to a file that can be mapped into their address spaces.

(3) The share wrapper sends a reference to the Arrow data to a \textit{SIPC} (Shared IPC) module, which extends the standard Arrow IPC implementation.  SIPC (like the unmodified version) is responsible for writing schemas, records, and dictionaries (as needed) to a sink, in this case an in-memory file.  SIPC will copy the schema to the sink as usual, but it will leverage new kernel support to share records and dictionaries without copying.

(4) SIPC sends the anonymous ranges of memory to a new kernel module, \textit{KernelZero}, that converts the anonymous memory to file-backed memory.  (5) KernelZero allocates new in-memory files and updates metadata in the process's address space to indicate that the specified range corresponds to a section of the new file. (6) KernelZero transfers ownership of previously anonymous memory to new in-memory files.  This transfer does not involve copying actual data, and afterwards both the process's address space and the in-memory file will point to the same physical memory pages.

(7) KernelZero returns identifiers for the new files and offsets corresponding to the de-anonymized ranges.  (8) SIPC writes references to the new de-anonymized files to the SIPC sink.  A SIPC file will be much smaller that an Arrow IPC file because it has references to the data instead of the actual data. This \textit{de-anonymization} technique enables \zc{} to avoid copying data on the write path (\textbf{Challenge 4}).

For nodes in a non-trivial DAG, it will be common to have processes that are both consumers and producers of Arrow data, and some operations may produce overlap between the input and output.  Examples include selecting a subset of columns, slicing rows, concatenating tables (along either axis).  When SIPC reads inputs, it records the locations where it maps input data into the address space.  Upon later writes, SIPC recognizes addresses corresponding to input ranges.  This enables \textit{resharing}: SIPC writes references to input files to the output stream instead of copying the data within the node (\textbf{Challenge 5}).

Resharing is sometimes possible with filtering and sorting too, but this is more challenging because inputs and outputs will overlap at fine-granularity (\ie{}, rows).  For regular encodings, \zc{} will unfortunately need to copy the data. For dictionary encodings, however, SIPC uses a \textit{dictionary sharing} technique; references to input dictionaries are written to outputs, and only columns of dictionary lookup codes must be copied. Consequently, dictionary encoding will often be useful for \zc{} even if there are no repeated strings in a column (the standard use case for dictionary encoding).

\subsection{Sharing-aware Resource Management}
\label{sec:design-rm}

The Resource Manager is responsible for tracking dependencies of intermediate data to the actual physical data, caching user-annotated intermediate data of loader nodes, and making scheduling and eviction decisions based on dependency information and memory usage.

\subsubsection{Dependency Tracking}

The RM track dependency information through SIPC.
With resharing, intermediate data is represented as virtual Arrow tables referencing physical memory.  Reference details are very relevant to caching decisions (\eg{}, it may be necessary to delete outputs from multiple sandboxes to free up a physical memory with multiple references to it). We cannot control the user code generating outputs, but SIPC inspects outgoing Arrow data and collects sharing information on behalf of the RM.  This \textit{IPC inspection} technique allows the RM to make informed eviction decisions regarding eviction and garbage collection (\textbf{Challenge 6}).

\subsubsection{DeCache}

The RM caches the deserialized data of specific loader nodes in DeCache, removes duplicated loads of the same Parquet source, and manages the contents of DeCache.

\zc{} provides generic loader codes that deserialize specified Parquet data to Arrow. DAG nodes can either provide custom code or use provided loader code. Using such codes indicates caching of the deserialized data generated by them and loader nodes that load already-cached data are not run and their children nodes' dependencies are redirected to the corresponding cache entry by the RM. When multiple DAGs rely on the same inputs, multiple nodes may map the same deserialized inputs (generated by loader nodes) into their address spaces. This \textit{deserialization sharing} avoids duplication of in-memory data across different DAGs (\textbf{Challenge 2}). Loader nodes and their outputs are managed as a deserialization cache (DeCache) so that DAGs starting at different times can still use the same inputs. 

Different DAGs may wish to deserialize the same data with or without dictionary encoding on certain columns.  In this case, different loader nodes will be used to create each representation (\eg{}, shows.parquet is deserialized with and without dictionary encoding in Figure~\ref{fig:arch}a).

The RM manages DeCache contents. Regular node sandboxes (and their outputs) are normally freed upon DAG completion, but DeCache sandboxes and outputs are preserved by the RM. Under memory pressure, the RM first evicts DeCache contents to free up space (``RM:uncache'' in Figure~\ref{fig:arch}a). 

\subsubsection{Eviction Mechanisms}
\label{sec:zero-copy-design}

The RM manages memory resources and is responsible for evicting in-memory data under memory pressure. Figure~\ref{fig:arch}a shows four actions (labeled with the ``RM:'' prefix) that the RM can perform.  First, the RM decides when memory should be allocated to start running new sandboxes (\textit{RM:alloc}) (the RM acts as a scheduler, deciding which node should receive the allocation). Second, the RM can perform three types of eviction action (\textit{RM:uncache}, \textit{RM:rollback}, and \textit{RM:limitdrop}) to free up memory as needed.  Uncaching DeCache entries and rolling back DAG progress both involve deleting completed sandboxes and their Arrow outputs. In the latter case, the node will need to be re-executed later so that the DAG can eventually complete.

Swapping, on the other hand, doesn't require rollback of completed nodes, but is tricky to be performant. A naive way is to rely on kernel swap; however, this could be suboptimal as the kernel might swap out intermediate data that will be consumed by nodes that will soon be scheduled to run. The kernel swaps in the order of LRU and altering such order with our knowledge of dependency is challenging due to limited kernel support for specifying what data in particular should be swapped out.  We thus borrow a technique, \textit{limit dropping}, from an early version of Senpai~\cite{meta-memory-offloading}.  With this approach, a container's memory limit is dropped to trigger swap.  In our case, in-memory files produced by a container are counted towards the container's memory limit, so the RM can select specific intermediate Arrow data to swap to disk. In order to retain control over intermediate data after a node finishes running, we allow the process in the container to exit upon node completion, but retain the container itself until the whole DAG completes (\textbf{Challenge 3}).

The RM has two mechanisms for evicting a non-cache node's output: \textit{rollback} and \textit{limit dropping}. The cost of deleting outputs depends on the latency of the function that generates the outputs and the cost of swapping depends on the size of the outputs. Thus, the RM adopts \textit{adaptive eviction}, which adaptively deletes or swaps the outputs of a function based on the ratio of its latency to the output sizes.  The threshold should be tuned offline and should depend on throughput of the swap device (\textbf{Challenge 3}).

\beforesect
\subsubsection{Admission and Eviction Policy}
\label{sec:policy}

The RM uses a fixed straightforward admission control that allows new sandboxes to be created when the available memory (not reserved by existing sandboxes) can satisfy the memory requirement of a node.  When multiple nodes are waiting for memory allocations, the RM assigns priority in depth-first order (\ie{}, the closest to finishing a DAG), as completing DAGs that are nearly finished enables deletion of all intermediate data for that DAG, freeing resources for other DAGs.

Admission control has the potential to cause deadlock if intermediate data has exhausted all system memory and all DAGs are waiting for memory to make progress; the intermediate data may not be releasable until DAG completion.  Even without deadlock concerns, too much intermediate data in memory could reduce the opportunity for more parallelism in DAG execution. 
Thus, the RM performs evictions using the knowledge of sharing details to free up memory as necessary. The RM chooses between memory-freeing actions as follows. First, the RM uncaches DeCache entries with no active references, if any. Then, the RM evicts the outputs of nodes with the lowest priority (as described based on depth) by adaptive eviction. Outputs are evicted one by one until the available memory is larger than the memory requirement of the node scheduled to run next.




==> tex/eval-extra.tex <==
\section{Evaluation (Extras)}
\label{sec:eval-extra}


\subsection*{Evaluation Plan}

1. Scheduling experiments - do we have time to discuss more on it? Current plan - 1 plot of percentage of overcommitting and 1 plot of other eviction techniques

2. Macro Benchmark - Let's see what it will look like.

3. The deduplication technique - The plan is to do this with Macro Benchmark, but do you have any better idea to evaluate it separately? Deserialization cache is a special case that is evaluated in 4.5

\subsection{Effect of Number of Threads}
\input{fig-tex/eval_thread}

Question: How many threads should we use in our experiments? This is more like a experiment to decide what parameter to use in later evaluation. And we find out that using the default setting (num of physical core, which is 32 in this case) is better.

Figure~\ref{fig:TODO} shows the effect of number of threads during a load workload. The load function loads 0.5\GB\ parquet file into 4\GB\ Arrow in-memory format with a number of parallel threads. The default is the number of hardware cores and is 32 on our machine. Then the Arrow in-memory format is then output to shmem. This step is always single-threaded.

For both baseline and \framework\, when the working set is much larger than the available memory, using more threads performs similer or slightly better than using one thread. When the working set is similar or smaller than the vailable memory, using more threads performs much better. We thus use the default number of threads which is the number of hardware cores in the rest of evaluation.

\subsection{Parallel Execution}
\input{fig-tex/eval_parallel}

Question: How \framework\ performs better because of the lower working set due to no copy.

\framework\ at most halves the working set size when executing functions that outputs Arrow tables. Figure~\ref{fig:eval-parallel-load-v2}(a) shows the results of running as many parallel load functions as possible. The function loads 0.5\GB\ parquet file into 4\GB\ Arrow in-memory table format and then outputs 4\GB\ Arrow IPC format of the table. \framework\ runs out of memory and starts to use swap space after 10 parallel executions while baseline starts to use swap at 7. Even after that, \framework\ performs at least 100\% faster than baseline due to the lower working set size. Figure~\ref{fig:eval-parallel-load-v2}(b) is the number of swaps during the workload, proving that we start to swap later and swap less.

Figure~\ref{fig:parallel-compute} shows the results of running as many computation-heavy functions as possible. The function loads 1GB data and does a series of operations: filter by rows, add and transform a few columns and then sort by rows. The entire workload triggers few swaps. We can see that with a function that is computation heavy and generates less output and runs entirely in memory, our benefit is lower, until baseline runs out of memory and starts to swap.

\yfnote{The current way of measuring swaps, that is counting major page faults, cannot be applied to the above workload with low or no swaps counts, as there will always be a small number of major page faults no matter swapping or not, and if swap count is very small, this noise becomes significant. I can't think of any better way of measuring, so maybe we don't show swap count for this workload that really incurs no swaps for \framework\ and only a little more at the right side of the graph for baseline?}

Figure~\ref{fig:eval-parallel-two-v2}(a) shows the results of running above two functions sequentially as a instance and running as many instances as possible. The results are similar to Figure~\ref{fig:parallel-parallel-load-v2} except for both \framework\ and baseline runs out of memory earlier (at 6 and 8) due to the memory consumption of the second computation function. Figure~\ref{fig:eval-two-v2}(b) shows the number of swaps during the workload.


\subsection{Scheduling}
\input{fig-tex/eval_schedule}

\yfnote{I don't know how to draw conclusions from current results. I think I need to run different sets of workloads. I will try to describe below.}

We want to answer (1) which overcommit percentage is better and (2) which eviction method is better with no overcommit.

Figure~\ref{fig:schedule-overcommit} runs the same workload as is Figure~\ref{fig:parallel-combine} with \framework\ with different overcommit percentages. Though there is no all-time best overcommit percentage, overall no overcommit is close to the best and lower overcommit is often better.

Figure~\ref{fig:schedule-active-eviction} also runs the same workload as is Figure~\ref{fig:parallel-combine}, but with different eviction methods. When reaching memory limit and there are schedule-able functions, ``No Active Eviction'' does nothing and wait for currently running functions to finish and free up memory (no deadlock in this workload). ``Active Swap'' manually swaps out currently unused outputs in shmem using instrumented fadvise. ``Active Delete'' deletes currently unused outputs and re-run corresponding functions (this is probably not a good idea especially in longer chains). When scheduling functions, depth-first method is used in all cases to free outputs more quickly and avoid deadlock. The conclusion is indecisive. All three policies work similarly, with ``Active Delete'' a little worse.

Comments: 

1) It is a little bit surprising that even 110\% overcommit starts to perform worse with a larger number of functions to schedule. This is probably also due to the fact that I am running identical workloads and their memory usage pattern is the same.

2) With no overcommit, it seems that doing nothing when facing memory limit and no deadlock is good enough. I will run another set of workloads that causes deadlock and add policies that do nothing when no deadlock and only swap/delete a minimal amount to make the dag make progress.

\subsubsection{A More Complicated Case}

Figure~\ref{fig:schedule-complicated-eviction} runs the same workload as in Figure\ref{fig:add-column}, each chain containing 10 functions and 1 to 20 chains are run.

In this workload, no matter how we prioritize functions, deadlock could happen. Thus we introduce three new eviction methods other than those shown in Figure~\ref{fig:schedule-active-eviction}. When reaching memory limit and there are schedule-able functions, ``Overcommit Once'', ``Delete Once'', and ``Swap Once'' wait for running functions to finish and only takes action on deadlock, where no progress can be made. Then, ``Overcommit Once'' simply issues one more function to run and let the kernel do swapping to make space for that function. ``Swap Once'' manually swaps out temporarily unused outputs to make space for running one more function. ``Delete Once'' deletes temporarily unused outputs (approximately outputs with lower time to generate are deleted first) to make space and rerun corresponding functions later to regenerate these outputs.

We can see that ``Delete Once'' and ``Active Delete'' performs much better. This is partially because functions in this workload runs fast, so the overhead of re-running functions is low. ``No Eviction'' deadlocks at 50 functions. Note that ``No Eviction'', ``Delete Once'', and ``Active Delete'' works with no swap space and the performance is similar to that in this graph. As ``Active Delete'' reruns much more functions than ``Delete Once'', we conclude that ``Delete Once'' is overall a better policy.

Figure~\ref{fig:schedule-complicated-overcommit} shows the performance of different overcommit percentages. No overcommit is still preferred.

Comments:

1) It seems that deleting only when necessary is the best strategy. I will run another set with longer function execution time to see if this is always true. Running this set of experiments is taking way more time than I expected.

==> tex/eval-macrobenchmark2.tex <==
\beforesect
\subsection{Workload Mix}
\label{sec:macrobenchmark}

We now evaluate how much each of \zc{}'s features contributes to overall performance for more complicated mixes of workloads.  In particular, we randomly generate five DAGs for each of the four packages in Table~\ref{tbl:macro-workload}, for 20 DAGs total.  Each DAG starts by loading a random Parquet file containing 1-4~GB of numerical data, stored across 4 columns.  How frequently different DAGs use the same inputs will affect DeCache performance; we tune repetitiveness so that about half of the DAGs share input with others (this is approximately the repetitiveness for the median Redshift cluster over the course of a week~\cite{Renen-24-Redshift}).

\begin{table}[tp]

\caption{{\bf DAGs in Workload Mix}.}

\begin{tabular}{l|l|l}
Name              & Library & Memory Usage              \\ \hline
Matrix Mult       & Numpy   & changing                  \\
Linear Regr & Scikit  & decreasing                \\
Col Append 1  & Pyarrow & increasing (w/ resharing) \\
Col Append 2  & DuckDB  & increasing               
\end{tabular}
\label{tbl:macro-workload}
\end{table}

All the DAGs are sequential chains (no branchout), and code as randomly generated for each nodes as follows.  \textit{Matrix Mult}: numpy is used to multiple the input table by a matrix to produce an output with the same number of rows and N columns (selected randomly between 1 and 10).  Some numpy data (including in this case) can be converted to Arrow data without a copy given both represent numbers consecutively in memory.  \textit{Linear Regr}: scikit-learn is used to perform a linear regression on the input data.  We randomly choose half the columns as features and one other column as the label.  The node splits the table into even-sides train/test sets.  A linear regression model is trained on the training data, then used to add a prediction column to the test data, which is used as the node's output.  \textit{Col Append 1}: PyArrow computes 4 new columns via simple operations over existing columns, horizontally concatenates the new columns to the input table (as for Figure~\ref{fig:schedule-long}a), and returns the result.  This naturally leads to resharing opportunities.  \textit{Col Append 2}: this is similar to the Col Append 1 pattern, but the projection adding the columns in implemented via a SQL query executed by DuckDB. Though DuckDB reads Arrow data without copy, a copy is required to transform a DuckDB table to an Arrow table to produce the output, so this workload type does not present resharing opportunities.



\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/eval_macro_tp_v2.eps}
    \vspace{-0.6cm}
    \caption{\textbf{Performance of Workload Mix}.
        The x-axis is the number of parallel DAGs. The y-axis is the throughput.
        % \if 0
        % The black line is baseline and others are \zc{} variants. \zc{} variants with the DeCache are marked in blue and others red. \zc{} variants with Adaptive Eviction are marked in solid lines and others are in dashed lines and uses \textit{kswap} that relies on kernel swapping to resolve deadlocks. %but does uncache unused DeCache entries if applicable. 
        % Baseline also uses \textit{kswap}.
        % \fi
        }

        
    \label{fig:macro}
\end{figure}

We generate two versions of the workload, with chains of depth 2 (so one loader node followed by one computational node) or 10.  N client threads (varied from 1-9) run as fast as possible, each submitting one DAG at time to the system.

Figure~\ref{fig:macro} shows the results.  \zc{}, with all features enabled, outperforms the baseline by 1.5-1.7$\times$ for short DAGs and 1.6-9.5$\times$ for long DAGs (depending on parallelism).  We observe that zero-copy writes (provided by SIPC) always provide significant benefits, whereas the DeCache only provides significant benefits for short DAGs and eviction only provides significant benefits for long DAGs.  The reason is that loading represents a bigger fraction of the work for short chains, so caching load output with the DeCache is especially helpful.  However, the DAGs are short enough so that there is little need for eviction features to rollback or swapout of intermediate progress.  In contrast, for long DAGs, loading is a relatively insignificant portion of the total work, but the ability to rollback or swapout progress on some DAGs to resolve deadlocks and make space for other DAGs so that they can make faster progress is essential.

Together with all the components, Kelvin is a robust, highly performant system under a variety of scenarios.

==> tex/extra/background.tex <==
\subsection{Linux Background (OLD)}

\subsubsection{Linux Memory Management}

\subsubsection{Virtual Memory}

Linux uses virtual memory in memory management. Virtual memory abstracts the details of physical memory from user-space processes, providing a mechanism for protection and controlled data sharing between processes. Each process has its own virtual address space and each memory access uses a virtual address, which is then translated to physical address by the page table, each entry in which corresponds to one physical page. Physical memory is divided into pages, typically 4KB in size. Each physical page can be mapped by one or more virtual pages, realizing data sharing between processes.

Virtual memory is divided into virtual memory areas. Each virtual memory area describes properties, such as permissions and backing device of a contiguous chunk of virtual memory.


\subsubsection{Anonymous Memory}

Memory not backed by any filesystems is called anonymous memory. Processes in Linux allocate anonymous memory implicitly by stack growing and explicitly by using \texttt{mmap} system call. Anonymous pages are not shareable between unrelated processes (processes with no parent/children/sibling relationships). Under memory pressure, anonymous pages can be swapped out, leaving a swap entry instead of a physical page number in its corresponding page table entries.


\subsubsection{Tmpfs Filesystem}

Tmpfs is a filesystem which keeps all of its files in virtual memory, living completely in the page cache and optionally on swap. Tmpfs files are like files on normal filesystems. They can be mapped by different processes, thus achieving data sharing.

The data of each file in tmpfs is represented by a series of physical pages. Each file has an array of entries, each entry corresponding to a physical page. If the page is swapped out, a swap entry replaces the physical page in the array, similar to what happens in a page table.

\subsubsection{Linux Details}

\textbf{Virtual Memory Management.}
A process's virtual memory space's managed by \texttt{struct mm\_struct}, or mm. An mm contains several virtual memory area, or \texttt{struct vm\_area\_struct}, or vma. A vma describes a contiguous virtual memory range and is either file-backed or swap-backed. Swap-backed vma's memory range contains anonymous pages, while file-backed ones contain file-backed pages. The backing device and offset information is recorded in vma to correctly fault pages in and swap pages out.

When no swapping or faulting is necessary (under no memory pressure and page table entries are valid), memory access doesn't need to go through mm and vma. Given a virtual memory address to be accessed, one walks the page table to find the corresponding page table entry which points to the physical page that contains the data.

Under memory pressure, physical pages from the start of lru queues (each cgroup has a set of lru queues for anonymous pages and file-backed pages and the ratio to evict from is a configurable parameter) are evicted from memory. Dirty anonymous pages needs to be swapped out to swap space to keep the data. When swapping anonymous pages, a swap entry is first allocated which records the swap space information and the offset into the swap space, then all the vma's that map the page are found by (incredibly complicated) reverse mapping data structures in the page. Then the correct page table entry is found and the swap entry replaces the physical page number in that page table entry. After all mappings are replaced with the swap entry, the anonymous page can be safely swapped.

When a memory access finds empty info or swap entry in a page table entry, it needs to fault the page in using the mapping and offset information recorded in the corresponding vma.

Each mm has a lock to protect itself and all its vma's. New memory allocation that adds and/or modifies vma information requires write lock, while page faults that reads vma information requires read lock.


\textbf{Cgroup Memory Controller.}
Control groups, usually referred to as cgroups, are a Linux kernel feature which allow processes to be organized into hierarchical groups whose usage of various types of resources can then be limited and monitored. Cgroup's memory controller supports reporting and limiting of process memory, kernel memory, and swap used by cgroups.

Each page in memory is either file-backed or swap-backed. File-backed pages are pages from files on regular permanent devices. They are charged to the cgroup whose process first loads them into memory (the page cache). Even if these pages are then shared among processes from different cgroups, only the first process is charged. The cgroup is discharged when the pages are evicted from memory. When these pages are brought into memory again, the loader then is charged.

Swap-backed pages includes anonymous pages and shmem file pages, as when they are evicted from memory, to prevent data loss they need to be written into the swap space on a permanent device. Swap-backed pages are created in memory and charged to the creator. Same as file-backed pages, sharing doesn't affect the charges of swap-backed pages. Different from file-backed pages, when swap-backed pages are evicted from memory, the owner is discharged for memory usage and charged for swap usage. Further, when they are brought back into memory, if their owner cgroup still exists, the owner is discharged fro swap usage and charged for memory usage no matter who the loader is. If the owner cgroup is removed at the time of load from swap, the loader is charged instead.

When cgroups are removed, their charges for memory are moved to their parent cgroups. Their charges for swap are not updated. When swapped pages are loaded, the recorded information for removed cgroups are discarded and the loader is charged, as described above.

==> tex/extra/bauplan.tex <==
\subsection{Data pipelines as DAGs}
\label{sec:dags}



\subsection{Bauplan architecture}
\textit{Bauplan} is a platform for declarative data pipelines over data lakes \cite{10.1145/3650203.3663335}. Users express transformations as straightforward Python functions with the signature $f(dataframe(s)) \rightarrow dataframe$\cite{10.14778/3407790.3407807}:

\addvspace{\baselineskip}
\begin{lstlisting}[columns=fullflexible,language=Python,caption=Fig.~\ref{fig:dag} DAG with Bauplan syntax]
@bauplan.model()
@bauplan.python('3.10', pip={'pandas': '2.0'})
def final_table(
    # reference to its parent DAG node
    data=bauplan.Model('source_table') 
):
   # transformation logic here
   my_final_df = data.do_something()
   return my_final_df

@bauplan.model()
@bauplan.python('3.11', pip={'pandas': '1.0'})
def training_data(
    data=bauplan.Model('final_table') 
):
   training_df = data.do_something()
   return training_df
\end{lstlisting}
\addvspace{\baselineskip}

The DAG structure is \textit{implicitly} expressed through function inputs, and reconstructed by the platform when the code is submitted; as for the relevant runtime properties, a simple decorator allows to express the desired Python interpreter and dependencies\footnote{The actual runtime details are beyond the scope of this paper, but Bauplan solves transformation independence through fast SOCK-like containerization \cite{216031}.}. 

The declarative nature of both pipeline topology and compute environments leaves the underlying optimizations to the platform, which compiles user code to chained, containerized functions and provides the required data operations over S3 / the wire. In particular, an optimal FaaS runtime should co-locate (whenever possible) related functions in the same host, to increase resource utilization and considerably shorten the feedback loop when compared to non data-aware FaaS (Section~\ref{sec:dags}). Our research question can therefore be succinctly asked as: \textit{how can fully separate processes efficiently share large dataframes}?

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/dag.jpg}
    \caption{Interleaving of compute (EC2) and storage (S3) in a data pipeline, modelled as a Directed Acyclic Graph (DAG): the responsibility of the data scientist is to write functions that transform the original data artifact (the source data) in intermediate and then final dataframes for downstream consumption.}    
    \label{fig:dag}
\end{figure*}



==> tex/extra/implementation.tex <==
\section{Old Design}
\label{sec:design}

\subsection{OpenLambda for DAG}
\label{sec:OL}

\yfnote{Maybe you can write a better general description of OL here...}

We instrument OpenLambda to recognize dependencies between functions in a DAG and reference tracking between Arrow IPC outputs of functions and the underlying physical data (shmem files generated by \framework) they depend on.

Based on policy, OpenLambda has several options under memory pressure. Without swap space, OpenLamdbda only schedule functions when the available memory is larger than the required memory of the function, and deletes outputs of finished functions if no progress can be made and re-run the functions later. With swap space, OpenLambda can manually swap out certain outputs from shmem to make room for new functions under memory pressure, or simply schedule functions that cannot fit in the memory and let the operating system to swap when necessary.

To manually swap out certain outputs from shmem, we keep the cgroup of finished functions and zero the cgroup memory limit of the generator function's process' cgroup and reset it to the original value for later swap in, utilizing the kernel behavior that swap-backed files' memory and swap usage are always charged to the creator cgroup until the cgroup is deleted.


\subsubsection{Deserialization Cache}
\label{sec:cache}

OpenLambda provides a common load function that loads parquet file from permanent storage and emits Arrow IPC format in shared memory, which is cached for any function that references the file to use. We call this cache Deserialization Cache. In one DAG execution, OpenLambda identifies functions that loads the same parquet file, execute the load function only once for the file, and let the dependant functions of these load functions depend on the same Arrow IPC output. 

Moreover, when there is no memory pressure, outputs of the common load function are not deleted when there are no active references (other outputs are deleted immediately after no active references). This enables functions from other DAGs coming later that loads the same parquet file to refer to the outputs. Thus, we eliminates duplicated loads from the same DAG as well as from other DAGs.

Under memory pressure, outputs of the common load function without active references are deleted in first priority.

OpenLambda also provides common load functions with advanced parquet loading options such as the \texttt{read\_dictionary} option which constructs dictionary encoded columns in Arrow tables from parquet files directly. Outputs generated by the same function with same parameters are considered the same and thus later loads are deduplicated.

\subsection{Share Manager}
\label{sec:reshare}

In Arrow IPC library, we build a Share Manager that tracks the source shmem files (generated by \framework) mapped by the input of the function. When generating Arrow IPC outputs, for any data buffer from the tracked input source, Share Manager records the input source and offset in the IPC output without transferring/copying the data. Share Manager also records the referencing relationship between outputs and the underlying physical data for OpenLambda's reference tracking which is helpful when freeing the data and making deleting and/or swapping decisions under memory pressure.

Special care needs to be taken for slicing arrays with offset buffers, e.g. string array. Arrow string arrays are composed of a bitmap, a data buffer that contains all the bytes of all the strings in this array, concatenated, and an offset buffer that contains the starting offset of each string in this array into the data buffer. Unmodified Arrow generates new offset buffers as it is designed to copy data anyway. To avoid this copy, when the sliced buffer originates from function input which means sharing is applicable, we could reuse the entire offset buffer (and the corresponding value buffer if applicable) and record the sliced offset in IPC metadata to reconstruct the sliced array with the entire buffers and the offset value without generating any new data.

Bitmaps with null values will also be re-generated when sliced for all kinds of arrays including arrays without offset buffers. One can apply similar approach to eliminate the copy but since bitmaps are very small compared to the data size and copies only occur when it contains null values, we simply allow this small copy to take place.

\subsection{DeAnon Design}
\label{sec:deanon}

\framework\ receives request for moving a virtual memory range of anonymous memory which cannot be accessed by other process to a specified shmem file. \framework\ traverses the page table to get the pages from the virtual memory region. For each page, \framework\ modifies the metadata of the page, the shmem file, and the virtual memory area the page belongs to, so that the page appears to belong to the shmem file and the virtual memory area appears to be a file mapping to the shmem file. After this step, the calling process can still access the data in the moved region, and other processes can map to the shmem file to access the data in the normal posix style. 

\yfnote{Actually, in the Arrow IPC case, we don't want the calling process to have shared write access to the shared region as following writes would propagate to the already written IPC data. But this would mean to change all the flags of related vma's and is too hard (and unnecessary in our controlled use case) to do, so I don't plan to do it.}

\subsubsection{Direct Swap}
\label{sec:direct_swap}

When the working set is larger than available memory, pages could be swapped out. In this case, \framework\ finds swap entries instead of pages after walking the page table. A naive way is to swap in the pages and follow the previous routine, but swapping is slow even if the swap space is on a fast NVMe device. Instead, \framework\ directly inserts the swap entry to the shmem file to let the entry belong to the file, and modifies the metadata of the swap space and the page table entry accordingly. This way we don't need to swap in pages during the de-anonymizing process and greatly improves performance when swapping occurs. The evaluation of this technique is in \sref{sec:direct-swap}.

\yfnote{I don't know if I should name this technique Direct Swap, or if I should name it. I am desperately incapable of naming...}

\subsubsection{Details}

\framework\ exposes two interfaces: \texttt{new\_file()} allocates a shmem file to receive anonymous memory in the future and \texttt{deanon(file\_id, addr, len)} to move the anonymous memory in \texttt{[addr, addr+len)} to the shmem file referred by \texttt{file\_id}.

\texttt{deanon()} first grabs the write lock of the process's mm, then split/merge the affecting vma's to have one vma containing exactly the range of memory to de-anonymize. Then the vma's backing is changed to the target shmem file, and we then traverse the page table and change each physical page in the range to be backed by the shmem file. If we meet a swap entry in the page table, we move the swap entry to the shmem file and mark the swap entry shmem-file-backed. The shmem file's metadata is changed accordingly so that it appears to contain these pages moved in.

\yfnote{The following is for internal reference. Not 100\% confident. I have solved every problem that I have seen, but I cannot guarantee there are no other problems. Other known issues are - deanonymized memory cannot be deanonymized again, and deanonymized memory cannot already be shared by other processes (shared anonymous mapping).}
There is an interval in this process that we go beyond (break?) kernel assumptions of its data structures, that is after the vma's metadata is changed and before the metadata of each page is changed. But (at least in the kernel version I use (5.15)) this entire process is not affected by other processes/threads faulting in and swapping out pages. First, faulting cannot happen as we grab the write lock. Swapping of pages that has been changed to shmem-file-backed can proceed as usual, but for these pages we have already come back to kernel assumptions. Swapping of pages that has not yet been changed to shmem-file-back cannot happen as the vma has been changed to shmem-file-backed and removed from the reverse-mapping data structures so the mapping in this vma cannot be located and unmapped. Thus the page will keep this mapping until it is changed to shmem-file-backed and pages with mapping cannot be swapped. So this entire process can be done without being interrupted by other processes/threads.








